Measuring Issue Ownership using Word Embeddings

Sentiment and topic analysis are common methods used for social media monitoring. Essentially, these methods answers questions such as, "what is being talked about, regarding X", and "what do people feel, regarding X". In this paper, we investigate another venue for social media monitoring, namely issue ownership and agenda setting, which are concepts from political science that have been used to explain voter choice and electoral outcomes. We argue that issue alignment and agenda setting can be seen as a kind of semantic source similarity of the kind "how similar is source A to issue owner P, when talking about issue X", and as such can be measured using word/document embedding techniques. We present work in progress towards measuring that kind of conditioned similarity, and introduce a new notion of similarity for predictive embeddings. We then test this method by measuring the similarity between politically aligned media and political parties, conditioned on bloc-specific issues.

==> left-news.tex <==
\begin{itemize}
\item Aftonbladet
\item Arbetarbladet
\item Dala-Demokraten
\item Folkbladet
\item ETC
\item Arbetaren
\item Flamman
\item Bang
\item Offensiv
\item Proletären
\end{itemize}



==> nativist-news.tex <==
\begin{itemize}
\item Nordfront
\item Samhällsnytt
\item Fria Tider
\item Nya Tider
\item Samtiden
\end{itemize}

==> right-news.tex <==
\begin{itemize}
\item Dagens Industri
\item Dalabygden
\item Hallands Nyheter
\item Axess
\item Svensk Tidskrift
\item Hemmets Vän
\item Dagens Nyheter
\item Göteborgs-Posten
\item Helsingborgs Dagblad
\item Nerikes Allehanda
\item Sydsvenskan
\item Upsala Nya Tidning
\item Expressen
\item Svenska Dagbladet
\item Smålandsposten
\item Norrbottens Kuriren
\end{itemize}

